Control of Magnetic Microrobot Teams for Temporal Micromanipulation Tasks

In this paper, we present a control framework that allows magnetic microrobot teams to accomplish complex micromanipulation tasks captured by global Linear Temporal Logic (LTL) formulas. To address this problem, we propose an optimal control synthesis method that constructs discrete plans for the robots that satisfy both the assigned tasks as well as proximity constraints between the robots due to the physics of the problem. Our proposed algorithm relies on an existing optimal control synthesis approach combined with a novel sampling-based technique to reduce the state-space of the product automaton that is associated with the LTL specifications. The synthesized discrete plans are executed by the microrobots independently using local magnetic fields. Simulation studies show that the proposed algorithm can address large-scale planning problems that cannot be solved using existing optimal control synthesis approaches. Moreover, we present experimental results that also illustrate the potential of our method in practice. To the best of our knowledge, this is the first control framework that allows independent control of teams of magnetic microrobots for temporal micromanipulation tasks.

==> Introduction.tex <==
\IEEEPARstart{O}{ver} the years, tremendous advancements have been made in lowcost fabrication of microscale parts. However, assembly and packaging of these homogeneous microscale parts to realize a heterogeneous functional microsystem account for a substantial fraction of the cost of commercial products.Due to the small sizes of objects micro-assembly operations are not suitable for manual handling. However, most of the efforts to automate micro-assembly operations meet with the unique challenges in object handling due to the unfamiliar microscale physics.  We have identified following factors that makes microassembly very challenging:

\textit{Automation}: Most of the micro-assembly operations require automation to be performed since the physics at microscale pose unique challenges for human operators. Autonomous microrobots capable of handling small objects are more suitable for these operations.   

\textit{Cost}: A major obstacle in commercialization of  microsystems is their cost. The high cost of microassembly and packaging which account for as much as 60\% to 90\% of total manufacturing cost of microsystems is regarded as one of biggest obstacles in commercial viability of microsystems. That also limits the widespread use of microsystems in commercial products. A micro-assembly station that is capable of performing operations in a cost-effective fashion would potentially revolutionize the field.  

\textit{Accuracy}: The assembly of microscale parts require the accuracy on the order of nanoscale because of size scale we have to deal with. This accuracy cannot be achieved with manual handling of parts. Precision of robotic microassembly operations largely depend on the quality of the actuation and associated control arrangements. 

\textit{Parallelization}: The throughput of the system depends on the maximum number of  parallel operations that  can be done in a particular instant. Use of  a swarm of microrobots to handle multiple parts can improve the throughput of the operation significantly. 

\textit{Flexibility}: Making a rigid assembly line for a certain product is very expensive since it cannot be reused with the change in the design of the product in the light of product upgrade or introduction of new product. Using mobile robots for microassembly operations can provide the flexibility of operation since they can be reprogrammed to do different tasks. 

\textcolor{blue} A multi robot army that can operate independently can potentially be used for parallel microassembly by moving individual components at the target location with high precision. We have developed a 11 $\times$ 11

To develop an army of autonomous microrobots to perform an efficient high throughput assembly operations we have to solve the temporal problem where all the robots have to synchronize their movements. The robots have to move to certain locations with respect to the others at a certain time instant. In this paper, we have developed a planning algorithm that not only avoid obstacles but also ensure the synchronization of the movement of the robots. 

==> LTLPlanning.tex <==
%Planning part: DUKE:\\
% \section{LTL Motion Planning}
Control synthesis for mobile robots under complex tasks, captured by Linear Temporal Logic (LTL) formulas, build upon either bottom-up approaches when independent LTL expressions are assigned to robots \cite{kress2009temporal,kress2007s,bhatia2010sampling} or top-down approaches when a global LTL formula describing a collaborative task is assigned to a team of robots \cite{chen2011synthesis,chen2012formal}, as in this work. Common in the above works is that they rely on model checking theory \cite{baier2008principles,clarke1999model} to find paths that satisfy LTL-specified tasks, without optimizing task performance. Optimal control synthesis under local and global LTL specifications has been addressed in \cite{smith2010optimal,smith2011optimal,guo2013revising, guo2013reconfiguration,guo2015multi} and \cite{kloetzer2010automatic,ulusoy2013optimality,ulusoy2014optimal}, respectively. In top-down approaches \cite{kloetzer2010automatic,ulusoy2013optimality,ulusoy2014optimal}, optimal discrete plans are derived for every robot using the individual transition systems that capture robot mobility and a Non-deterministic B$\ddot{\text{u}}$chi Automaton (NBA) that represents the global LTL specification. Specifically, by taking the synchronous product among the transition systems and the NBA, a synchronous product automaton can be constructed. Then, representing the latter automaton as a graph and using graph-search techniques, optimal motion plans can be derived that satisfy the global LTL specification and optimize a cost function. As the number of robots or the size of the NBA increases, the state-space of the product automaton grows exponentially and, as a result, graph-search techniques become intractable. Consequently, these motion planning algorithms scale poorly with the number of robots and the complexity of the assigned task.  

To mitigate these issues, we combine an existing optimal control synthesis algorithm with a novel technique that aims to reduce the state-space of the product automaton satisfying at the same time the LTL statement. Specifically, given transition systems that abstract robot mobility, we create trace-included transition systems that have smaller state-spaces than the original ones. To do so, we first compute shortest paths among locations that the robots definitely need to visit in order to accomplish their assigned tasks. These locations can be determined by inspection of the temporal logic formula. Locations that are included in these shortest paths comprise the backbone of the trace-included transition systems. Then, we introduce states in the constructed transition systems through a sampling-based approach until the resulting discrete abstractions are expressive enough to generate motion plans that satisfy the assigned task. Then, discrete plans are synthesized using graph search methods applied on a synchronous product automaton. Finally, we show through simulation studies that our proposed algorithm can address large-scale planning problems that cannot be solved using existing optimal control synthesis approaches. A preliminary version of this planning approach is presented in \cite{kantaros15asilomar} applied to an intermittent communication problem. 

%Furthermore, instead of considering obstacle-free environments as in \cite{turpin2014capt,panagou2014decentralized,zavlanos2008dynamic}, in this work we assume that robots navigate in complex environments. Complex environments are considered in \cite{turpin2013_rss, turpin2014_AR}, as well, where the task assignment problem is solved so that collision-free trajectories that connect every robot to its assigned task are generated. Navigation functions for driving a mobile network to a desired configuration while avoiding collisions with the environment have also been employed \cite{loizou2008_TRO}. In this work, collision avoidance with the environment and between the robots is guaranteed by construction of the discretized abstraction of the workspace captured by transition systems.


==> MobileMicrorobotPlatform_old.tex <==
\begin{figure*}[h] 
\centering
\subfloat[]{\label{fig:coil1}\includegraphics[width=0.48\textwidth]{figures/coil11.png}}
\hspace*{0.2cm}
\subfloat[]{\label{fig:coil2}\includegraphics[width=0.48\textwidth]{figures/coil21.png}}
\\
\subfloat[]{\label{fig:coil3}\includegraphics[width=0.48\textwidth]{figures/coil31.png}}
\hspace*{0.2cm}
\subfloat[]{\label{fig:coil4}\includegraphics[width=0.48\textwidth]{figures/coil41.png}}

\caption[]{Sequential operations of three robots to finish an assembly task: (a) Initial position of the robots and parts; (b) Robot 1 moves to manipulate the part 1 to the desired location, (b) Robot 1 retracts after placing the part 1 to the desired location while Robot 2 to take over the task, (c) Robot 2 and Robot 3 take the parts 1  and 2 to the desired positions, (d) Finally, Robot2 and Robot 3 finish the assembly task.}
\label{fig:coil}
\end{figure*}
\label{sec_intro}

We have developed platform with multiple microrobots actuated independently with the use of local magnetic filed. We have developed an array of planar microcoils each with a dimension of 5 mm $\times$ 5 mm. Each planar microcoil has a winding width of $177.8$ $\mu m$, an out-of-plane winding thickness of $177.8$ $\mu m$, and a winding spacing of $177.8$ $\mu m$ with $10$ turns. Each winding is rectangular in shape for the ease of fabrication.  Each coil is capable of generating a local magnetic field that is dominant only in it's vicinity. The coils and the traces are separated by a thick insulation layer of about $1.5$ mm which provides sufficient isolation. The current in each coil can be controlled through a custom control unit which can switch the direction and control the magnitude of current. Each coil is designed to carry a maximum current of 1 A.

Robot: The robot considered for the experiments in a $3.125$ mm diameter and $0.79$ mm thick neodymium disc magnet. This magnet is of grade N52 and magnetized through its thickness. 

Robot movement physics and action set: The motion of the robot can be controlled by controlling the currents in the coils in the vicinity of the robot. 

End effectors

Figure~\ref{fig:coil} shows an assembly task with two parts accomplished by three robots. Every robot has an end effector that helps to push a part to a desired location (Figure~\ref{fig:coil1}). 
The assembly task starts with the Robot 1 pushing the Part 1 to the desired location in the workspace. Robot 1 backs off after taking the part 1 to the desired location. Robot 2 then takes over the manipulation task by pushing the robot in towards the final destination where both parts will be assembled. At the same time, part 2 is pushed by the Robot 3 towards the desired location. Finally, both the parts are manipulated to finish the assembly task.

In order to accomplish the assembly tasks  efficiently, there has to be a temporal correlation between the movements of the robots. The efficiency of the manipulation tasks can be greatly increased only with a temporal planning between the robots.  This paper will achieve the temporal planning between the robots for effective completion of assembly tasks.  
